White Dwarf Pollution by Asteroids from Secular Resonances

In the past few decades, observations have revealed signatures of metals polluting the atmospheres of white dwarfs. The diffusion timescale for metals to sink from the atmosphere of a white dwarf is of the order of days for a hydrogen-dominated atmosphere. Thus, there must be a continuous supply of metal-rich material accreting onto these white dwarfs. We investigate the role of secular resonances that excite the eccentricity of asteroids allowing them to reach star-grazing orbits leading them to tidal disruption and the formation of a debris disc. Changes in the planetary system during the evolution of the star lead to a change in the location of secular resonances. In our Solar System, the engulfment of the Earth will cause the $\nu_6$ resonance to shift outwards which will force previously stable asteroids to undergo secular resonant perturbations. With analytic models and $N$--body simulations we show that secular resonances driven by two outer companions can provide a source of continuous pollution. Secular resonances are a viable mechanism for the pollution of white dwarfs in a variety of exoplanetary system architectures.

==> RESPONSE.tex <==
RESPONSE: We thank the referee for the very thorough report. We have made all of the changes that have improved the manuscript. We hope that the paper will be accepted for publication now. We outline our responses below.

Reviewer's Comments:

You aim to explain the excess of heavy elements observed in numerous white dwarf spectra by a continuous supply of asteroids, reaching star-crossing orbits through secular resonances with planets.

Globally, the goal of your article is clear and the argumentation is well documented. However, the precise mechanism involved (namely, the engulfment of an inner planet by the Star) remains elusively described. It is even omitted at some points of the article, where you seem to take the mass loss of the star as the main responsible for the shift of the secular resonance, contrary to the arguments used for the computations.

Moreover, I see three main weaknesses in the arguments presented. The first two concern the computation of a rate of mass supply from the numerical simulations (Eq. 19) and its comparison to values inferred from observations.
	1) The initial population of asteroids used for the numerical simulations is very different from what we would expect for a real system (you use a uniform distribution of a,e,I in given ranges). It is true that the real inner boundary of the Main Belt is used, but even inside the Main Belt, the distribution of asteroids is far from begin homogeneous.
	2) In order to distinguish the particular effect of the nu6 secular resonance, the initial population of asteroids is distributed inside a very narrow range of semi-major axes. This sample is thus designed to be perturbed by the nu6 resonance, and far from being representative of the whole asteroid belt. It is thus erroneous to estimate a global mass rate from the total mass of the Main Belt, as you do. It produces a very overestimated rate.   
	3) In the third section, you apply the Laplace-Lagrange equations to very heavy planets, and even to star companions with masses larger than the central body mass. Since the Laplace-Lagrange equations are first order with respect to the orbital perturbation, this holds only if this highly massive companion is very far away. However, you explore also ranges of semi-major axes in which the perturbation is comparable or even higher than the terms coming from the central body.
    

In my opinion, your article still brings interesting ideas and should be published, but I suggest a major revision. A moderate revision could be envisaged if you choose to remove the quantitative result (namely, the mass rate estimate). Please find below my comments and suggestions.

MAIN MODIFICATIONS
For points 1) and 2):
	- Descoping: remove the mass rate estimate (Eq. 19). The continuous flux obtained from the simulations (Fig. 4) is already interesting in itself. Naturally, the impact of the article would be diminished, since there will be no quantitative result. I find, however, that the qualitative description of your "pollution scenario" is interesting enough to be published.
OR
	- Redo simulations from a sample representative of the whole Main Belt (in order to be able to use its total mass). In this case, however, the specific role of the nu6 resonance would be indistinguishable from other effects.
OR
	- Redo simulations from a sample representative of the portion of Main Belt you are interested in, but then, estimate the mass rate from the mass of this portion only. If you think other secular resonances could have similar effects, then the maximum you could do in order to get a global estimate is to multiply the rate by their number (2, 3, 5?). In any case, you cannot generalise the rate to the whole Main Belt population.
    
RESPONSE: We have added a new section 2.2.1 where we simulate the actual asteroid belt distribution around the nu6 secular resonance during post-main-sequence (Earth is engulfed) and calculate a more realistic accretion rate. We note that this is a lower limit to the accretion rate since we are only considering asteroids from a narrow range of semi-major axes.

For point 3):
	- Check the range of semi-major axis over which the Laplace-Lagrange system gives relevant results and show only this portion in Figs. 5 and 6. At the very least, warn the reader about the qualitative nature of these curves, since the approximation used is very crude (or even wrong) for small semi-major axes of the stellar/planetary companion.
    
RESPONSE: We have removed 0.1 solar mass companion from Fig.7. We have warned the reader about the qualitative nature of these curves in the figure captions for Figs.6 and 7.

COMMENTS AND SUGGESTIONS
General remarks:
The “astronomical unit” is written in upper case characters all along the article. It is not a problem for me, but it should be noted that the IAU explicitly recommends to use lower case characters.

RESPONSE: We have corrected this.

Abstract:
- The portion “As a stat loses mass...to perturb previously stable asteroids.” should be removed. This is not the argument used in the article to justify the shift of the secular resonances. At the place of this portion should appear instead the two sentences currently placed below: “Changes in the planetary system...to undergo secular resonant perturbations.”

RESPONSE: We have corrected this sentence.

- The part “These asteroids become tidally disrupted and form a debris disc...” is not clear. It could be replaced by something like: “These asteroids reach star-grazing orbits due to the resulting eccentricity excitation, leading them to tidal disruption and the formation of a debris disc...”

RESPONSE: We have corrected this sentence.

- The sentence “This process occurs...binary star companion.” could be removed.

RESPONSE: We have removed this sentence.

Introduction:

First paragraph:
- The sentence “A total of 1000...” should be placed before the references, or a specific reference for this number should be added.

RESPONSE: We have corrected this.

- I would find it clearer to move the part “The stratification or diffusion timescales...than the white dwarf cooling time (Paquette et al. 1986)” just before the sentence “Accretion discs and pollution are observed at 30 Myr to 600 Myr...”. In this way, the two timescales are directly compared.

RESPONSE: We have corrected this.

Second paragraph
- The sentence “The currently favored pollution mechanism suggests that...” is vague. It should be stated that this tidal disruption occurs because of close encounter of the metal-rich bodies with the star.

RESPONSE: We have corrected this.

Third paragraph:
- For the process to be really adiabatic, the timescales should be very well separated. The adiabatic approximation is thus valid for semi-major axes well below 2000 au, not just “below”. The sentence could be slightly rephrased to incorporate this.

RESPONSE: We have corrected this.

Fourth paragraph:
- The sentence “Each resonance has a width, in semi-major axis, over which it operates.” is misleading. Actually, this applies only for mean-motion resonances. For secular resonances, the locations and widths depend strongly on (a,e,i), which makes them much harder to study. See for instance Knezevic et al. 1991.

RESPONSE: We have corrected this.

Fifth paragraph:
- The last two sentences (“Because of the...”) are unclear. If I understand correctly what you mean, they could be rephrased into something like: “If the planetary system undergoes major changes during the stellar evolution (for instance, if inner planets are engulfed by the star), the secular frequencies of the whole planetary system would be affected, resulting in a displacement of the location of secular resonances. On the other hand, the location of mean-motion resonances with the remaining planets would remain almost unchanged.”.

RESPONSE: We have corrected this.

Section 2.1

- In the sentence “Jupiter increases the precession...”, the words “apsidal precession frequency of Saturn” should be replaced by “mean apsidal precession frequency of Saturn”. Indeed, the precession frequency of Saturn actually contains harmonics of all the planets. However, the g6 term has a much larger amplitude, so it corresponds to its mean apsidal precession.

RESPONSE: We have corrected this.

- “The location of the nu6 resonance is found by calculating the location of the intersection of a test particle’s precession rate...” => “In this paper, the location of the nu6 resonance is estimated by calculating the location of the intersection of a test particle’s free precession rate...”

RESPONSE: We have corrected this.

Section 2.1.1
- It is crucial here to recall the basics of the theory you use: it is linear in e and i, and it gives the secular perturbation at first order to the orbital perturbation. It is important to keep it in mind all along the article (and especially in Sect. 3, where you apply it to a variety of different systems).

RESPONSE: We have corrected this.

- At Eq. 2, there is a missing nj.
Please check also in your program, I hope the mistake is only in the paper, otherwise you should redo your calculations.

RESPONSE: This is only a mistake in the paper, not in the code. We have corrected this in the text.

- In the last paragraph, you should replace “(See also Minton & Malhotra 2001)” by “See Laskar (1988) for further comparisons.” Indeed, Laskar (1988) made a whole table designed to such comparisons.

RESPONSE: We have corrected this.

- The remaining portion of the paragraph (from “Brouwer & van Woerkom obtained a more accurate...”) has no utility for the present work and should be removed.

RESPONSE: We have corrected this.

Section 2.1.2
- Please replace any occurrence of “precession rate of the asteroid” by “free precession rate”. As for Saturn above, this is quite different! This precession rate is often written g0 by authors, and it corresponds to the diagonal term of the Laplace-Lagrange matrix including the asteroid (Morbidelli & Henrard 1991, Milani & Knezevic 1990).

RESPONSE: We have corrected this.

- In more general theories, the location of secular resonances depends of a, e and i (Knezevic et al. 1991). Hence, as second sentence of this section, you should write: “In this linear theory in eccentricity and inclination, it is only function of the secular semi-major axis a”.

RESPONSE: We have corrected this.

- Equation (8): there is an inversion in the definition of the coefficient bar-alpha. It should be 1 for an inner perturber, and the ratio of semi-major axes for an outer one. Please check also in your program, I hope the mistake is only in the paper, otherwise you should redo your calculations.

RESPONSE: This is only a mistake in the paper, we have corrected this in the text.

- Last paragraph: please precise that you will first consider the case N=3 (Earth+Jupiter+Saturn), and after that N=2 (Jupiter+Saturn).

RESPONSE: We have corrected this.

Section 2.1.3
- “secular resonance with Saturn” => “secular resonance with the proper mode of Saturn”

RESPONSE: We have corrected this.

- The last sentences of this section are unclear and contain redundant information. They could be simplified into: “We use the observed inner and outer boundaries of the asteroid belt to produce this region, that is the range [2.1;3.5] au in semi-major axis. The observed inner boundary, created by the nu6 resonance, is consistent with our analytical model which places it at about 2 au.”

RESPONSE: We have corrected this.

Caption of Figure 1
- “free precession rate”

RESPONSE: We have corrected this.

- “Both Jupiter’s and Saturn’s orbital separation” => “the semi-major axes of Jupiter and Saturn”

RESPONSE: We have corrected this.

- There is a missing “of” in the last sentence of the caption.

RESPONSE: We have corrected this.

- In the figure, Jupiter and Saturn are inverted.

RESPONSE: We have corrected this.

Section 2.1.4
- You cannot call it a resonance width. You should replace it by something like “eccentricity excitation”, or “maximum eccentricity excitation”, otherwise this would be very misleading for readers. The computation of a resonance width requires a change of coordinates (taking the resonant angle as independent variable), and the computation of the ranges of orbital elements in which this angle librates. This is impossible to realise with your approach, since this model is intrinsically non resonant. Graphs similar to Fig. 2, however, give an idea of the location of secular resonances (but not of their width!).

RESPONSE: We have corrected this.

- The first two sentences of the section are redundant and can be removed.

RESPONSE: We have corrected this.

- “free precession rate”

RESPONSE: We have corrected this.

- In Eq. 11, there is a mistake of Laplace coefficient: (1) => (2)
Please check also in your program, I hope the mistake is only in the paper, otherwise you should redo your calculations.

RESPONSE: This is only a mistake in the paper, we have corrected this.

- As you indicated it, h_0 and k_0 are function of time. Then, how is defined e_max? Is it defined at a specific time? Or do you take only the term of Saturn? Or do you take the maximum of e_forced(t) (which consists in summing the absolute value of the coefficients)?

RESPONSE: We have removed the word maximum and just use forced eccentricity. The forced eccentricity is defined as when t->0.

- After Eq. 15, you should write at the end of the sentence “, obtained from the initial conditions of the planetary system”.

RESPONSE: We have corrected this.

- “Jupiter and Saturn with orbital separation of...” => “Jupiter and Saturn with semi-major axes of...”

RESPONSE: We have corrected this.

Caption of Fig. 2
- The eccentricity range shown seems to be a bit large compared to the very low-order theory used. You should decrease the vertical range or warn the reader in the caption (something like: “Our theory is not accurate for such high values of the eccentricities, but we show it as an indication”).

RESPONSE: We have corrected this.

- “The stellar mass loss shifts the nu6 resonance outwards due to this engulfment”. This sentence is particularly misleading. It is not the mass loss which shifts the resonance, but the engulfment of the Earth! This point is particularly important (see my very first comments). You should show the relative effects of the two mechanisms by plotting four curves instead of only two: 1) e_max for Jupiter+Saturn at present date, 2) e_max for Jupiter+Saturn at white dwarf stage, 3) e_max for Earth+Jupiter+Saturn at present date, 4) e_max for Earth+Jupiter+Saturn at white dwarf stage. I did it, and the resonance location (a_res/a_Jup) for cases 1)-2), and 3)-4) are nearly equal. This means that the shift of the secular resonance due to mass loss is negligible, and that the shift from your Fig. 2 is only due to the disappearance of the Earth.

RESPONSE: We emphasized in the caption that the mass loss in due to the engulfment of the Earth. We have kept just two curves, we had already did what you mentioned and there is no change, so we wanted to keep this figure simple as possible.

- Moreover, you should tell something about the amplitude of the shift. It is very small compared to the crude approximation of the dynamics given by your linearised analytical model. Remember that you make an error of some tenths of astronomical units in the location of the resonance, which is of the same order of magnitude of the shift. Still, I think that the mechanism you describe here is qualitatively interesting, because the shift could be much larger if a planet bigger than the Earth is engulfed.

RESPONSE: We have include information about the amplitude of the shift at the end of section 2.1.

- “...to undergo secular perturbation” => “...to undergo stronger secular oscillations of eccentricity”.

RESPONSE: We have corrected this.

- Could you add somewhere in the article (possibly in appendix) the complete set of parameters used to draw Fig. 2 (masses of the Sun, Jupiter, Saturn, Earth; the semi-major axes; and the resulting location of nu6)? In this way, interested readers will be able to redo the calculations.

RESPONSE: We have added table~1 with the complete set of parameters used to draw Fig. 2

Section 2.2
First paragraph:
- The sentence “do interact gravitationally with the planets...” is unclear. I suppose you treated asteroids as test-particles (zero mass), so they do not disturb the planets (but they are disturbed by the planets). Please clarify this.

RESPONSE: We have clarified this sentence.

- “The timescale for resonant perturbations […], whereas...”: interesting! This is rarely precised in the literature.

Second paragraph:
- Instead of “located at 2.1 au (Petit et al. 2001)" you should simply write “(2.1 au)”. The article by Petit et al. should be cited much before this point, for instance in the introduction, where you mention this value.

RESPONSE: We have corrected this in the text. We have cited Petit et al. 2001 in the fifth paragraph in the introduction.

- “Thus, we only simulate the region that we expect asteroids to be in.” => this is not true. The actual asteroid distribution is far from being uniform in these ranges of orbital elements (see my very first comments). I am convinced that if you run your simulation at current epoch, with the same initial distribution of asteroids, you will get also a lot of ejections and collisions with the Sun, (even if the Earth is present). In Knezevic et al. 1991, you can see the shape of the nu6 resonance in the (a,i) plane. Your distribution completely overlaps it.

RESPONSE: We have added a section 2.2.1 where we model the actual asteroid belt around the nu6 secular resonance during post-main-sequence (Earth is engulfed) and calculated a more realistic accretion rate.



Fourth paragraph
- “since the solar system is stable over long timescales” => “since the outer solar system is stable over long timescales (Laskar 1994)”

RESPONSE: We have corrected this.

Fifth paragraph
- “Since the asteroids in our simulations are non self-interacting point-particles” => could be removed.

RESPONSE: We have corrected this.

- The destabilisation of asteroids should begin as soon as the Earth is engulfed, that is, when the Sun is still a red giant. Many objects will thus be ejected or will collide with the star before it reaches its white dwarf mass and radius. You should say something about it, for instance comparing the timescale between Earth engulfment and the white dwarf state of the Sun (0.5 solar masses).

RESPONSE: We added a couple sentences on this.

Sixth paragraph
- It is true that the tidal disruptions for the 2:1 resonance in your model is overestimated, but it is also the case for the nu6 one (see my above comment about your initial distribution). However, the ratio of disruptions in the two cases are so different that your conclusions probably still hold.

RESPONSE: We have made this more clear.

Seventh paragraph
- You speak of tidal disruption (you even increase the radius of the star on this purpose) and of the creation of a disc of material, but you subsequently suppose that your asteroids are immediately swallowed but the star. I think you should point out that the asteroids could possibly be torn apart but remain in the form of a debris disc, forming a reservoir which could produce a steadier supply of heavy elements in the long run. The rate shown in Fig. 4 should thus be lower, but probably steadier.

RESPONSE: We have explained this near the end of the new section 2.2.1.

Eighth paragraph
- I find this whole paragraph very questionable, see my very first comments. (By the way, note that Debes et al. (2012) used the real distribution of Main Belt asteroids in order to compute their own estimate of the mass accretion rate.) Moreover, all the text from “Their conclusions suggest that at least 27%...” up to “...is the exponential diffusion timescale for calcium.” is useless for introducing your own estimate (Eq. 19). The values cited at the beginning of the paragraph would be enough.

RESPONSE: We have removed a portion of this paragraph from the next and placed the remaining part as the first paragraph in section 2.2.1.

Last paragraph
- I would not say that your numerical results agree with the analytic model. The main reason comes from the initial conditions you used (see my above comment). In my opinion, these numerical simulations cannot be used to confirm the analytic part, neither to compute a relevant mass accretion rate. However, the simulations do show very clearly that the nu6 resonance is much more efficient than the 2:1 MMR to produce Sun-crossing orbits.

RESPONSE: We just wanted to say that the shift found in our analytical model is seen in our numerical results. We have added figures 4 and 5 to deal with this issue. We have also made this more clear at the end of section 2.2.1.

Section 3
- See my general comments about the use of the Laplace-Lagrange equations for very massive and close planets.

RESPONSE: We warned the reader about the qualitative nature of these curves and we removed the low mass (0.1 M) companion from figure 8.

- “dynamics of the nu6 secular resonance location for...” => “displacement of the nu6 secular resonance for...”

RESPONSE: We have corrected this.

Section 3.1
First paragraph:
- “The value of 30 AU was based on the theoretical adiabatic expansion of the planet HR8799e.” I don’t agree. Since the initial mass of the star is 1.56 solar masses and that you still consider a white dwarf with 0.5 solar masses, the resulting semi-major axis is about 47 au, not 30. Can you explain this discrepancy?

RESPONSE: We have removed the information regarding HR 8799. Instead we emphasize modeling two regimes, less than and greater than the semi-major axis of Jupiter.

Moreover, you should precise that you will actually not study the case of HR8799e. As it is mentioned all along this article, the architecture of the planetary system makes vary the location of the secular resonances. In the HR8799 system, the presence of two outer massive planets (much more massive than Uranus or Neptune) could produce large changes in the eigenfrequencies of the system.

RESPONSE: We have corrected this.

Second paragraph:
- “precession rate”, “precession frequency” => “free precession rate”, “free precession frequency”

RESPONSE: We have corrected this.

Third paragraph:
- “If we assume that the asteroid has the same adiabatic location, ...” You should rephrase this sentence. Indeed, it is erroneous to consider a given location of the asteroid belt (before or after adiabatic expansion), because it should have been sculpted by the interaction with the planets well before the white dwarf stage. A clearer sentence could be like: “Let us consider an asteroid belt initially confined by the nu6-like secular resonance. Assuming that an efficient rate of disrupted asteroids is obtained whenever the asteroid belt is close enough to the star, the more massive the outer planetary companion, the larger its semi-major axis.”

Last paragraph:
- remove “and therefore be a potential mechanism of pollution” and add at the end of the paragraph: “and subsequent pollution of their atmosphere.”

RESPONSE: We have corrected this.

Section 3.2
First paragraph
- do you have a source for this 50% ?

RESPONSE: We have included a source.

- “wide-binary perturbation” => “perturbations by galactic tides for wide binaries”

RESPONSE: We have corrected this.

- add at the end of the paragraph: “for which none of these mechanisms are possible.”

RESPONSE: We have corrected this.

Second paragraph
- “Since these represent theoretical models only...may produce with dwarf pollution”. These two sentences are unclear. As above, a clearer way to put it is: “Assuming that an asteroid belt is initially confined by the nu6-like secular resonance, these models demonstrate that...”

RESPONSE: We have corrected this.

- Moreover, you should recall here the validity domain of your approximation: near-zero eccentricities and inclinations (of planet and binary), and very large distance of the binary (see my general comments about the use of the Laplace-Lagrange equations for very massive and close perturbers). “A wide variety of binary configurations” seems thus a bit optimistic.

RESPONSE: We have corrected this.

- How did you obtain your upper limit of a_binary = 1000 au? Is it related to the adiabatic approximation or the location of the nu6-like secular resonance?

RESPONSE: We change the upper limit to about 400 au. This value is related to the location of the nu6-like secular resonance.

Conclusion

First paragraph:
- “can lead to polluted white dwarfs” => “can be responsible for the presence of heavy elements in the atmosphere of white dwarfs”

RESPONSE: We have corrected this.

- The second sentence is pretty long and contains wrong sequence of verb tenses. Please rephrase this part.

RESPONSE: We have corrected this.

- At the end of the paragraph, add: “assuming the presence of an asteroid belt initially confined by a secular resonance, and the engulfment of an inner planet during the evolution of the star.”

RESPONSE: We have corrected this.

Second paragraph:
- this paragraph should be written in the introduction rather than in the conclusion

RESPONSE: We have corrected this.

Third paragraph:
- This paragraph has several weaknesses.
At first, the mass loss of the star is not the argument you used throughout this paper. Actually, the location of secular resonances drifts almost linearly with the mass loss (I checked it), as do MMR. Therefore, your scenario absolutely requires the engulfment of an inner planet.
Second, see my above comments about your estimate of the mass accretion rate.
Third, you should recall what differs between your model and the one by Debes et al. (2012) and Frewen & Hansen (2014), and why your results are more encouraging.

RESPONSE: We have corrected this.

Fourth paragraph:
- “whethersolar m the Solar System will have a polluted white dwarf” => “ whether the Sun will be polluted during its white dwarf stage”

RESPONSE: We have corrected this.

- “viable explanation” => “possible mechanism”

RESPONSE: We have corrected this.

- “There is strong evidence that there may not be just one...” => “There is probably not just one...”

RESPONSE: We have corrected this.

- “secular perturbations last longer than mean-motion perturbations” => Are you sure? What are your arguments? The flux coming from secular resonances seems to be higher, but from your article, we have no idea of the relative timescales involved.

RESPONSE: We have corrected this.

Fifth paragraph:
- Why do you focus only on the Kepler database?

RESPONSE: We have added more databases.

- The last sentence is misleading. Indeed, you suppose, in your pollution model, that the architecture of the exoplanetary system shares strong features with the Solar System: 1) two outer massive planets, 2) An inner asteroid belt truncated by a secular resonance 3) An inner planet which is engulfed during the stellar evolution 4) all the bodies on nearly circular and coplanar orbits. This is quite specific, so contrary to what is written, this should indicate that the presented results may have little implication for systems vastly different from ours! However, you could precise that mean-motion and secular resonances are expected to sculpt the architecture of any asteroid belt in exoplanetary systems, so the global mechanism presented in this article and in Debes et al. (2012) should be triggered (with more of less efficiency) in various planetary configurations.

RESPONSE: We have corrected this.

==> RESPONSE2.tex <==
RESPONSE: We thank the referee once again for another very thorough report that has further improved the manuscript. We have addressed the concerns of the referee and we outline our responses below.



Scientific Editor's Comments:
Editor
Comments to the Author:
Although I can see that progress has been made, there is still some way to go before your manuscript can be accepted for publication.  The reviewer still has several legitimate concerns - some major and some minor.  Please respond to the points raised and revise your manuscript accordingly.


Assistant Editor's Comments:
The text in several of your legends is still not legible; please enlarge this.

RESPONSE: We have enlarged several legends.



Reviewer's Comments:
Reviewer: 1

Comments to the Author
Thank you for your reply. In overall, I agree with the modifications you made, resulting in my opinion in a much better version of your article.

However, I still judge that this article is not ready for publication:
 - Your definition of e_forced still appears incomplete.
 
RESPONSE: Instead of using e_forced, we have used the maximum forced eccentricity which is given in equation 16.
 
 - Your simulations with uniform semi-major axis distributions occupy too much space in the article, given the small amount of information they actually bring.
 
RESPONSE: We have reduced the size of the section that describes the uniform semi-major axis simulations. We have also moved these simulations into section 2.3 called "Efficiency Comparison". 
 
 - The specific role of the shift of the nu6 secular resonance is still not assessed in your new simulation. The only rigorous way to prove its influence it is to redo the exact same simulation with the Earth included.
 
RESPONSE: We have redone the exact same simulation but with the Earth included. We compare these two simulations in section 2.4 where we have updated Figures 5, 6, and 7. Based on the results obtained from this comparison, we conclude that the shift in the secular resonance is due to the engulfment of the Earth.

I think these points can be easily taken into account. More generally, I also encourage you to adopt a critical position with respect to the suggestions from your reviewers: your laconic answers made me wonder sometimes whether you agreed or not with my comments and whether you understood what I meant.

Please find below the detail of my comments for the new version of your article. 

ABSTRACT
- "the location of a secular resonance" => "the location of secular resonances"

RESPONSE: We have corrected this sentence.

1 INTRODUCTION
FIRST PARAGRAPH
- "It takes about 20 Myr to reach a temperature of 25,000 K (Fontaine et al. 2001)." => could be removed, since these values are present in the next sentence.

RESPONSE: We have removed this sentence.

- "It is noteworthy that DA white dwarfs fall..." => "It is noteworthy that DA
(hydrogen atmosphere) white dwarfs are observed..."

RESPONSE: We have corrected this sentence.

- "fall in the range" => "are observed in the range"

RESPONSE: We have corrected this sentence.

- And what about the cooling ages for DB white dwarfs ? (You mention them in the next sentence.) If the cooling ages that you give are also representative of the DB population, you could removed the word "DA" in this sentence and introduce DA and DB only in the next one.

RESPONSE: We have removed the word "DA" in this sentence and introduced DA and DB only in the next one.

SECOND PARAGRAPH
- "which means pollution found in ”wide” binary systems could be caused by planetary debris" => "which means that this mechanism is inefficient for wide binary systems"

RESPONSE: We have corrected this sentence.

THIRD PARAGRAPH
- You should rather cite Veras et al. (2011) instead of Maoz (2016). Indeed, Veras et al. (2011) did a careful analysis of the problem, and the numbers they give are documented (contrary to Maoz).

RESPONSE: We have cited Veras et al. (2011).

- "at orbital radii well below 2000 AU" => I am still not satisfied with this sentence, which is not consistent with the mass-loss rate of 1e-04 that you give earlier in the paragraph. I am surprised that you cite Veras et al. (2013), who wrote instead that the adiabatic approximation holds for planets "within a few hundred au of their star". This seems to me more reasonable.

RESPONSE: We have corrected the criteria for the adiabatic approximation. We have cited the work from Veras et al. (2013) and have said that the adiabatic approximation is valid for objects within a few hundred au of their star.

- "the timescale for mass loss is longer than" => "the timescale for mass loss is much longer than"

RESPONSE: We have corrected this sentence.

SIXTH PARAGRAPH
- In my opinion, the whole paragraph beginning with "During adiabatic mass loss..." can be removed. All the ideas written here were already introduced in the previous paragraph.

RESPONSE: We have removed this paragraph.


2 SOLAR SYSTEM
- At the end of this paragraph, you should precise that even if Mercury and Venus will also be engulfed, you will here focus on the effects of the Earth engulfment.

RESPONSE: We have added a sentence on this at the end of the paragraph.

2.1 ANALYTIC MODEL
- "The nu6 secular resonance properties are affected by both Saturn and Jupiter" => "The nu6 secular resonance properties are mostly affected by Saturn and Jupiter"

RESPONSE: We have corrected this sentence.

2.1.1 EIGENFREQUENCIES
- "The eigenfrequency are" => "The eigenfrequencies are"

RESPONSE: We have corrected this sentence.

2.1.2 ASTEROID PRECESSION RATES
- last sentence : "the precession rate of the asteroid" => "the free precession rate of the asteroid"

RESPONSE: We have corrected this sentence.

CAPTION OF FIGURE 1
- "the free precession of Saturn's proper mode" => What do you mean here? Maybe: "Saturn's dominant proper mode"?

RESPONSE: We have corrected this sentence.

2.1.3 FORCE ECCENTRICITY
FIRST PARAGRAPH
- "The forced eccentricity is calculated at t=0." => The time "t=0" has no precise meaning here. By definition, the times are different during the main main-sequence stage and the post-main-sequence stage. I advise you to show instead the maximum forced eccentricity (sum of the absolute value of the coefficients appearing in h0 and k0).

RESPONSE: We have added a new paragraph at the end of section 2.1.4, where we discuss the derivation of the maximum forced eccentricity.


- "the eigenfrequency dominated by the proper mode of the ith planet" => Again, what do you mean here? Maybe: "the dominant proper mode of the ith planet?"

RESPONSE: We have corrected this sentence.

- The amplitudes eji of the orbital solution for the planets, appearing in Eq.15, also depend on the longitudes of perihelion of the planets. You do not seem to take them into account, though, and they don't appear in Table1... How do you choose them?

RESPONSE: We have chosen the present-day values for the longitudes of perihelion for the planets and we have included these values in Table1.

SECOND PARAGRAPH
- "the mechanism we describe here is qualitatively interesting" => The word "interesting" is a bit subjective... You could put instead: "the mechanism we describe here is still qualitatively relevant"

RESPONSE: We have corrected this sentence.

2.2 4-BODY SIMULATIONS
SECOND PARAGRAPH
- "To see the effects of the resonance shift" => I still strongly disagree with this. Your two simulations with uniform semi-major axis distribution do not show anything about the shift of the resonance. They can only be used as a hint that the nu6 secular resonance could be more effective to drive asteroids towards the Sun than the 2:1 mean-motion resonance with Jupiter, regardless of any mass loss or planet engulfment. If you definitely want to maintain these simulations inside the article, you should introduce a new subsection for it, called for instance "Efficiency comparison", in which you briefly discuss these results.

RESPONSE: We have incorporated a new section called "Efficiency comparison". We have also reduced the length of this section by moving the general description of the tidal disruption rate to the end of section 2.2 which generally describes the 4-body simulations for our efficiency comparison and the real asteroid belt.

- "The actual asteroid belt distribution is far from being uniform but we analyze this distribution..." => "The actual asteroid belt distribution is far from being uniform, so we analyze its actual distribution..."

RESPONSE: We have corrected this sentence.

FIFTH PARAGRAPH
- "The evolution timescale for the mass loss is around..." => Do you mean "the evolution timescale between the red giant and white dwarf stages"?

RESPONSE: We have rephrased the sentence as suggested.

- "we assume instantaneous engulfment" => according to your answer to my previous comment, you should maybe rephrase it as: "we assume that after the Earth engulfment, the Sun instantaneously shrinks to its white dwarf state"

RESPONSE: We have rephrased the sentence as suggested.

CAPTION OF FIGURE 3
- I still strongly disagree with the last sentence. See my comment about the second paragraph.

RESPONSE: We have removed the last sentence: "Thus, all of the tidal disruption events during the $\nu_6$ simulations occur on previously stable asteroids that have survived the process of stellar evolution."

CAPTION OF FIGURE 4
- "adiabatically" => "adiabatically shifted"

RESPONSE: We have corrected this sentence.

2.2.1 TIDAL DISRUPTION RATE FROM THE ASTEROID BELT
SECOND PARAGRAPH
- "that have the orbital properties of asteroids in the asteroid belt" => What do you mean? How did you choose them?

RESPONSE: We have made it more clear on how we selected the objects.

THIRD PARAGRAPH
- "We use an unbiased selection of objects from the MPC..." => This should figure earlier (see my previous comment), with a footnote containing the internet address. You should also explain how you made this selection.

REPONSE: We have moved "We use an unbiased selection of objects from the MPC..." to the second paragraph, and made it more clear on how we selected the objects.

- "which reinforces that this is caused by the shift in the secular resonance" => This is actually not so clear. The only way to show that these disruptions are due to the engulfment of the Earth is to redo this exact same simulation with the Earth included, and add the corresponding curve in Figure 5. Depending of the results obtained, it could also be interesting to have the same graph as Figure 6, but for the simulation including the Earth. If the simulation including the Earth shows indeed a much lower rate of tidal disruptions, then, the effect of its engulfment would be assessed.

RESPONSE: We have included the simulation where we assume  the Earth is not engulfed. We have added that simulation to Figure 5 (red-dotted line), which shows that the peak is left of the peak representing the engulfment simulation (red-solid line). Next we have added an additional panel in Figure 6, showing the initial distribution of the asteroids that were tidally disrupted and at what time. Comparing these two panels, there is a higher concentration of tidally disrupted particles in the engulfment simulation versus the no engulfment simulation.

FIFTH PARAGRAPH
- At Equation 17, the number you give is obtained by supposing that the asteroids are cubic! A better approximation is obtained by supposing that they are spherical, with a volume of 4/3*pi*R^3. Please redo your calculation. I obtain about 5e+05 g/s.

RESPONSE: We have redone our calculations to include spherical asteroids. Using the new rate determined by the difference in the tidal disruption rate between engulfment and no engulfment, we estimate the mass accretion rate to be about 2.5e+05 g/s.

- "they will be torn apart and form a debris disc with asteroidal composition, forming and eventually..." => "they will be torn apart, forming a debris disc with asteroidal composition, and eventually..."

RESPONSE: We have corrected this sentence.

- "we observe the shift of the secular resonance" => I do not agree. A real fiducial simulation would be the same simulation with the Earth included. This is the only way in my opinion to assess its role in this process.

RESPONSE: We have included Figure 5 which shows the tidal disruption rates for each simulation (Earth engulfment versus no earth engulfment). We also show the difference between the two rates. We conclude that this observed difference is due to the shift of the resonance.

3 EXOPLANETARY SYSTEMS
3.1 PLANETARY COMPANIONS
SECOND PARAGRAPH
- "dominated by the outer companion's proper mode" => can be dropped

RESPONSE: We have dropped the suggested phrase.

- "The free precession frequency of the test particle..." => This sentence can be dropped. It seems obvious to me that the two planets were included in the calculations.

RESPONSE: We have dropped the suggested sentence.

3.2 STELLAR COMPANIONS
THIRD PARAGRAPH
- The whole paragraph beginning with "The analytical model may provide..." can be dropped. These points are already detailed in the conclusion (which is the right place for them).

RESPONSE: We have removed the suggested paragraph.

4 CONCLUSIONS
FIRST PARAGRAPH
- "This occurs because..." => I would rather write "mainly occurs", because actually the proper frequencies of the planets change as well (but by a small amount if the engulfed planet is small).

RESPONSE: We have corrected this sentence.

SECOND PARAGRAPH
This ideas developed in this paragraph are pretty similar to what is written in the first one. It would be much clearer for the reader if you merge these two paragraphs. In my opinion, the only really informative sentence of this second paragraph is the last one.
- "We expect the process of asteroid perturbations..." => "From our numerical experiments, we expect the process..."

RESPONSE: We have removed the second paragraph, and added the corrected last sentence to the first paragraph. 

THIRD PARAGRAPH
- "be accreted by the white dwarf" => "be accreted by the white dwarf by this mechanism alone"

RESPONSE: We have corrected this sentence.

FOURTH PARAGRAPH
- "but we expect that a higher flux..." => "but for exoplanetary systems resembling the Solar System, we expect that..."

RESPONSE: We have corrected this sentence.

==> RESPONSE3.tex <==
RESPONSE: We greatly appreciate the helpful comments from the referee. We have dealt with all of the concerns and we hope that the paper is now acceptable for publication. We outline below our responses to each of the points raised.

Reviewer's Comments:
Reviewer: 1

Comments to the Author
In my opinion, the new version of your article is much clearer and your results are more robust. I only have some minor comments:

Paragraph between Eqs. 15 and 16 and Table 1: You previously used \bar{\omega} to note the longitude of perihelion (see Eq. 10). Please use the same convention everywhere.

RESPONSE: We have used \bar{\omega} to denote the longitude of perihelion throughout the paper.


Equations 16 and 17: There is a mistake here. The values of h_0 and k_0 cannot be maximum at the same time (if one is maximum, the second is zero, as shown by Eqs. 13 and 14). Hence, the maximum forced eccentricity (Eq. 16) is equal to the right-hand side of Eq. 17 (sum of the absolute values). Consequently, Eq. 17 is wrong and it should be removed. Please also correct Fig. 2.

RESPONSE: We have fixed the calculation of the maximum forced eccentricity and updated Fig.2.

Section 2: Since they present the results of the N-body simulations, I think Sects. 2.3 and 2.4 should be two subsections of Sect. 2.2.

RESPONSE: We have made Sects 2.3 and 2.4 into subsections of Section 2.2.

Section 2.4, paragraph 3: the the => the

RESPONSE: We have fixed this.

Section 2.4, paragraph 4: After the sentence "At later times...", you should add something like: "This shows that their eccentricity growth is indeed due to secular effects, contrary to the highly unstable population represented by yellow points in Fig. 6."

RESPONSE: We have added the suggested sentence at the end of the paragraph.

Figure 6: Some colours are quite hard to distinguish. You should avoid yellow and/or use thicker lines (or full circles).

RESPONSE: We have changed the color bar to avoid using yellow and we have used full circles.


Figure 7: Could you fit a constant to the red dotted line (difference of the results given by the two models) and add it to the graph? This would be your continuous supply of asteroids coming from the nu6 resonance. The level of this curve (about 2e-4 I guess) should be used to compute the accretion rate (Eq. 19) instead of 5e-4.

RESPONSE: We have added a constant best-fit to figure 7 and have recalculated the accretion rate (now Eq. 18) with the rate 2e-04.


==> RESPONSE4.tex <==
RESPONSE: We thank the referee for the helpful report.  We have dealt with all of the concerns and we hope that the paper is now acceptable for publication.

Reviewer's Comments:
Reviewer: 1

Comments to the Author
Dear Authors,

Thank you for your revised version. Please note that there is still a missing "bar" at the omega character above Eq. 16.

RESPONSE: We have corrected this.

Apart from that, I do not see any further reasons to delay the publication.
